Connecting What to Say With Where to Look by Modeling Human Attention Traces

We introduce a unified framework to jointly model images, text, and human attention traces. Our work is built on top of the recent Localized Narratives annotation framework [30], where each word of a given caption is paired with a mouse trace segment. We propose two novel tasks: (1) predict a trace given an image and caption (i.e., visual grounding), and (2) predict a caption and a trace given only an image. Learning the grounding of each word is challenging, due to noise in the human-provided traces and the presence of words that cannot be meaningfully visually grounded. We present a novel model architecture that is jointly trained on dual tasks (controlled trace generation and controlled caption generation). To evaluate the quality of the generated traces, we propose a local bipartite matching (LBM) distance metric which allows the comparison of two traces of different lengths. Extensive experiments show our model is robust to the imperfect training data and outperforms the baselines by a clear margin. Moreover, we demonstrate that our model pre-trained on the proposed tasks can be also beneficial to the downstream task of COCO's guided image captioning. Our code and project page are publicly available.

==> Localized Narratives/text/0.abstract.tex <==
\begin{abstract}
% We introduce two novel tasks for vision-and-language research: (1) controlled visual trace generation and (2) combined caption and trace generation. 
We introduce a unified framework to jointly model images, text, and human attention traces.
Our work is built on top of the recent Localized Narratives annotation framework~\cite{pont2019connecting}, where each word of a given caption is paired with a mouse trace segment. 
We propose two novel tasks: (1) predict a trace given an image and caption (i.e., visual grounding), and (2) predict a caption and a trace given only an image.
Learning the grounding of each word is challenging, due to noise in the human-provided traces and the presence of words that cannot be meaningfully visually grounded.
We present a novel model architecture that is jointly trained on dual tasks (controlled trace generation and controlled caption generation).
To evaluate the quality of the generated traces, we propose a local bipartite matching (LBM) distance metric which allows the comparison of two traces of different lengths.
Extensive experiments show our model is robust to the imperfect training data and outperforms the baselines by a clear margin.
Moreover, we demonstrate that our model pre-trained on the proposed tasks can be also beneficial to the downstream task of COCO's guided image captioning. Our code\footnote{Code: \href{https://github.com/facebookresearch/connect-caption-and-trace}{github.com/facebookresearch/connect-caption-and-trace}} and project page\footnote{Project page: \href{http://pages.cs.wisc.edu/\~zihangm/connect\_caption\_trace}{http://pages.cs.wisc.edu/{\raise.17ex\hbox{$\scriptstyle\sim$}}zihangm/connect\_caption\_trace}} are publicly available.

%our flexible model architecture can be easily extended to perform controlled image captioning task\licheng{remind: update this statement.}, and it achieves state-of-the-art results on the COCO dataset.
% \zihang{Zihang}
% \ning{Ning}
% \tberg{Tamara}
% \amy{Amy}
\end{abstract}

==> Localized Narratives/text/1.intro.tex <==
\section{Introduction}

% Key reference: 
% localized narratives~\cite{pont2019connecting}
% gaze, vision, language~\cite{yun2013studying}
% gaze in egocetric vision~\cite{fathi2012learning}
% ~\cite{li2013learning}
% ~\cite{li2018eye}
% ~\cite{xu2015gaze}
% attention in image captioning
% show, control and tell~\cite{cornia2019show}
% show and tell~\cite{xu2015show}
% babytalk~\cite{lu2018neural}
% referring expression
% ~\cite{yu2016modeling}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.46\textwidth]{Localized Narratives/figures/title_figure.png} 
% \vspace{-10pt}
\caption{The three vision-and-language tasks, as illustrated on a single example from the Localized Narratives dataset. The first and third depicted tasks are novel.}
\label{fig:three_tasks}
% \vspace{-10pt}
\end{figure}
% Figure link: https://www.figma.com/file/pkgjSqGgpNXZoaOsMBKw3g/Localized-Narratives?node-id=0%3A

%\amy{1st paragraph: Introduce the high-level motivations and research areas of the paper -- visual grounding and image captioning}
%As researchers have developed increasingly 
The development of powerful models and algorithms within computer vision and natural language processing proceeded along distinct trajectories with only occasional overlap until recently. 
However, ideas from these two fields are gradually converging, with a focus on building multi-modal models, particularly for aligning visual and language stimuli~\cite{ViLBERT_NeurIPS_2019,tan2019lxmert,Su2020VLBERT,chen2019uniter}.
The goal of these models is to mimic humans' extraordinary abilities to compress information and translate it across modalities.
Several joint or combined visual recognition and natural language understanding tasks have emerged as natural tests of these vision-and-language models' capabilities.
\emph{Image captioning} asks a model to identify and localize the key scene elements in an image and describe them in natural language form.
\emph{Visual grounding}, and specifically \emph{phrase localization}, asks a model to solve the reverse problem: given a natural language query, identify the target object(s) of the query in the image.
\emph{Controlled image captioning}, first introduced in~\cite{cornia2019show}, combines the two tasks. 
Here, an external user is asked to specify which parts of the image they want described and in what order (e.g., by providing an ordered sequence of bounding boxes). 
The output captions are therefore explicitly grounded in the image. 
One application of this line of work is automatically generating localized descriptions of images for visually impaired users on social media services.
%, so that they may be more immersive when participating in social conversations, viewing their friends' photos, and reading the news. 
This removes the need to rely on human-written ``alt'' text, which is often missing in web images~\cite{Bigham_2006}. 
%Controlled captioning also gives users more fine-grained control over image understanding, allowing them to drill down into smaller regions of an image. 


%\amy{2nd paragraph: Describe at a high-level the previous research in this area and methods of approaching the task.}
Vision-and-language models share common components and techniques.
Image captioning architectures are typically composed of two modules: an image encoder, which ingests and interprets an image, and a language model decoder, which generates a natural language caption~\cite{xu2015showDenseCap,Huang_2019_ICCV}. 
Visual grounding models first identify the key components of the image (i.e., bounding box proposals) and query (i.e., which words or phrases to focus on), extract features from each, and then correlate them to predict the referred-to object~\cite{Rohrbach_2016,Hu_2016a,plummer2015flickr30k,yu2016modeling}.
Architectures for both tasks often rely on attention~\cite{xu2015showDenseCap,Deng_2018_CVPR,Huang_2019_ICCV,ViLBERT_NeurIPS_2019}, a mechanism inspired by the human visual system~\cite{Rensink_2000,Corbetta_2002}.
%that compresses an image or natural language phrase into a saliency map so the model can focus computation on the most important entities and features. 
Researchers have also designed more complex models that can do both caption generation and grounding. 
For example, \cite{Mao_2016_CVPR} and~\cite{yu2016modeling} can both generate an unambiguous description of a specific object or region in an image and automatically select an object given a referring text expression.
%Perhaps the most popular way of learning attention is to regard it as a latent variable in vision and language tasks~\cite{xu2015show,You_2016_CVPR}.
%These implicit attention maps are meant to teach models to focus on similar regions of images as humans do, although recent work demonstrates that this is not always the case.~\cite{das2017human}.

%\amy{3rd paragraph: Point out what it's missing in the previous approaches}
Despite these advancements, existing image captioning and visual grounding models cannot jointly generate longform, natural language captions \emph{and} dense, word-level visual groundings.
This is because existing image captioning datasets only provide short captions with sparse groundings at the noun level (Flickr30k Entities~\cite{plummer2015flickr30k}) or phrase level (Google RefEx~\cite{Mao_2016_CVPR}, Flickr30k Entities~\cite{plummer2015flickr30k} and Visual Genome~\cite{krishna2016visualgenome}).
To address these limitations,~\cite{pont2019connecting} introduced the Localized Narratives dataset, in which annotators were asked to describe an image with their voice while simultaneously drawing a mouse trace over the region they are describing.
This annotation framework provides rich, longform image captions and dense visual grounding in the form of a mouse trace segment for each word.
The work in \cite{pont2019connecting} incorporates the annotated mouse trace to aid in standard image captioning and controlled image captioning tasks.
However, it does not investigate the reverse problem of directly predicting the mouse trace or explore the connections between caption generation and trace generation.

%\amy{4th paragraph: Introduce our proposed approach, and how it fits in with the current research.}
In this paper, we take a step beyond~\cite{pont2019connecting} by requiring models to directly predict the trace, which is analogous to a fine-grained and temporally grounded log of human attention. 
Besides \emph{controlled caption generation}, where a model generates a caption guided by the given ordered trace from~\cite{pont2019connecting}, we further introduce two challenging new tasks: \emph{controlled trace generation}, where a model must densely localize each word from a natural language caption in an image, and \emph{joint caption and trace generation}, where a model is only given an image and must act as an annotator in the Localized Narratives protocol.
% These tasks are described in detail in Section~\ref{subsection:define_3tasks}.
There tasks are shown in Fig.~\ref{fig:three_tasks}.
% and are described in detail in Section~\ref{subsection:define_3tasks}.
{The task of predicting the trace is meaningful in two ways. First, a point-wise trace is a straightforward means for representing eye gaze. Learning the trace (independent of specific use cases) could be variously useful, and this is made possible by the efficient collection scheme described in \cite{pont2019connecting} which does not rely on expensive gaze trackers. Second, this form of annotation yields ``weakly-labeled'' word-level grounding. We demonstrate that such ``weak'' word-to-trace alignment could offer benefits for some important vision and language tasks. Besides, the predicted trace can provide a better explanation than most attention-based image captioning approaches.}
To evaluate the generated traces, we propose a novel evaluation metric, local bipartite matching (LBM), to compare two traces of arbitrary length.
% described in Section~\ref{subsection:eval_metrics}.
We present a flexible new transformer-based model architecture that is trained in parallel on controlled caption generation and controlled trace generation. 
%We specifically design the model to take advantage of the mirrored nature of the two tasks, by sharing parameters and learning from the joint training of the other task. 
The model also incorporates a symmetric cycle loss to improve the quality of the generated caption and trace. 
% The full model architecture is described in Section~\ref{subsection:mirrored_transformer}.
In addition to the three tasks mentioned above, we show that our approach can benefit downstream tasks by pre-training on our proposed tasks before fine-tuning for the downstream setting.

%In this paper, we take advantage of the rich image captions and dense visual grounding provided by the Localized Narratives dataset in order to address the current limitations of vision-and-language models. 
% in order to study the tight connections between vision and language. 
% in order to better understand the relationship between vision and lanuage.
%Based on the multi-modal annotations from Localized Narratives, we propose ...
% We begin by proposing a pair of challenging new tasks: \emph{controlled visual trace generation}, where a model must densely localize each word from a natural image caption in an image, and \emph{combined caption and trace generation}.
% Our tasks go a step beyond~\cite{pont2019connecting} by requiring models to directly predict the trace, which is analogous to a fine-grained and temporally grounded map of human attention.
%It also involves the interaction between three modalities (image, caption, and trace), compared with traditional vision-and-language tasks which only involve two modalities.

% We hope that ... // put this language in the conclusion.

%\amy{5th paragraph: Finally, summarize the paper's contributions}
To summarize, we make the following contributions:
\begin{itemize}
    \setlength\itemsep{0em}
    \item  We introduce two novel tasks: ($i$) controlled trace generation and ($ii$) joint caption and trace generation.
    \item We present a novel mirrored transformer model architecture (\modelName), which is jointly trained and evaluated on three vision-and-language tasks.
    %: controlled trace generation, controlled image captioning, and joint caption and trace generation.
    \item We design an evaluation metric to address the challenge of computing the distance between two traces of different lengths.
    \item By jointly learning from the mirrored trace generation task, our proposed method benefits the downstream task of guided caption generation on the COCO dataset.
\end{itemize}







==> Localized Narratives/text/2.related_work.tex <==
\section{Related Work}
% how our proposed two tasks are novel 
% how our model is novel 
% jointly learning from the mirrored trace generation

%{\noindent \textbf{Image caption and visual grounding }}
\paragraph{Image Captioning} 
Image captioning is typically formulated using a generative model, creating descriptions in textual space given the input image via CNN-to-RNN/LSTM/Transformer~\cite{vinyals2015show, chen2015mind, karpathy2015deep, cornia2020m2}.
An increasingly common addition to this basic architecture is a visual attention
mechanism which typically produces a spatial map that identifies the specific image
region(s) most relevant to the current word prediction task~\cite{xu2015show, anderson2018bottom}.
However, the learned spatial attention may not well align with human attention~\cite{das2017human}. 
To model attention more directly, controlled image captioning was first introduced in \cite{xu2015showDenseCap}.
It requires the user to provide a sequence of bounding boxes in the image and outputs the image caption in the same order, describing the objects in those bounding boxes. 
The authors in \cite{pont2019connecting} adjusted the task by using an annotator's mouse trace for the control. %We follow the same setup in this work. 

% \cite{anderson2018bottom} introduced bottom-up attention mechanism for image captioning. 
% Recently, transformer-based methods have been widely used for image captioning \cite{Huang_2019_ICCV, decoupled_emnlp, entangled_transformer, unified} and further advanced the performance. 

%  Referring Expression, Flickr30K, DenseCaption, Localized Narratives

% Previously, the drawbacks in these approaches were due to dataset limitations.
% Existing image captioning datasets either lack grounding supervision (COCO Captions~\cite{chen2015microsoft}, Conceptual Captions~\cite{sharma2018_conceptual_captions}, Stanford Visual Paragraphs~\cite{krause2016paragraphs}) or only provide grounding at the noun level (Flickr30k Entities~\cite{plummer2015flickr30k}) or short phrase level (ReferIt~\cite{ReferIt_2014}, Google RefEx~\cite{Mao_2016_CVPR}, Flickr30k Entities~\cite{plummer2015flickr30k} and Visual Genome~\cite{krishna2016visualgenome}).
% These datasets supply phrase-level grounding in order to make the results of image captioning models more interpretable and easier to evaluate~\cite{Mao_2016_CVPR}.
%These datasets have limited lengths and are biased toward nouns~\cite{pont2019connecting}.

\paragraph{Visual Grounding} 
The task of visual grounding is to localize a region described by a given text query.
Researchers have introduced multiple datasets to tackle this problem, such as RefCOCO~\cite{yu2016modeling}, Google RefEx~\cite{Mao_2016_CVPR}, Flickr30K~\cite{plummer2015flickr30k}, and DenseCap~\cite{johnson2016densecap}.
State-of-the-art approaches~\cite{yu2018mattnet, yu2017joint, liu2017referring, zhang2017discriminative} treat visual grounding as selecting the most matched box to the input text query.
However, the input query is typically short (the average length of captions in RefCOCO is 3.5 words) and the grounding is sparse (each query corresponds to just a single box).
By contrast, our work focuses on denser word-to-region grounding.
 
% \cite{johnson2016densecap} introduced a new dense captioning task and predicted object detection bounding boxes together with the image caption. 
% \cite{Mao_2016_CVPR} and~\cite{yu2016modeling} jointly generate referring expressions and localize them in an image, but only for a single object at a time. 
% These methods also produce sentence fragments, rather than complete sentences or paragraphs. \cite{ma_ECCV2020} and~\cite{zhou2019grounded} produce complete sentence captions with word-level groundings, but they do not ground every word and do not ground relationships. In this work, our novel task can ground each word in the sentence and predicts both the grounding and caption at the same time.

\paragraph{Localized Narratives} 
As described above, image captioning datasets only provide image-sentence pairs without the spatial localization of words. Visual grounding datasets only provide sparse region-sentence mapping. 
Recently, Localized Narratives~\cite{pont2019connecting} was proposed, which offers dense word-region alignment for each full caption.
This dataset was collected by recording annotators' voice and mouse traces simultaneously when describing the image content.
The three modalities of image, trace, and caption significantly expands the scope of how we can connect vision and language.
While~\cite{pont2019connecting} only addressed a single task of controlled captioning, we introduce two more novel and challenging tasks, i.e., controlled trace generation, and joint caption and trace generation.
At first glance, these three tasks as shown in Fig.~\ref{fig:three_tasks} appear separate; however, we propose a unified framework using a mirrored transformer to jointly model all three tasks.
%, and enable the two tasks to interact with each other.
% , which improves standard image captioning and controlled image captioning tasks. 
% In this paper, we propose two novel tasks to generate trace, which \cite{pont2019connecting} didn't investigate.

% While most of these work take image features as input and decode caption, we propose a novel mirrored transformer architecture which supports three input modalities with shared weights. 


% {\noindent \textbf{Controlled Image Captioning. }}Gaze, language, vision
% attention in image captioning,
% controlled image captioning

% % {\noindent \textbf{Joint Image Captioning And Visual Grounding Methods. }}


% % I don't think VQA is relevant [Ning]
% % {\noindent \textbf{Visual Question Answering. }} Stuff on VQA.

% % Potentially talk about joint training

% In this work, we address both. Working on localized narratives, dense alignment between visual region, trace segment, and words, our model is 

% We present a flexible new transformer-basedmodel architecture that is trained in parallel on trace-guidedcaption generation and caption-guided trace generation. Wespecifically design the model to take advantage of the mir-rored  nature  of  the  two  tasks,  by  sharing  parameters  andlearning from the joint training of the other task. The modelalso  incorporates  a  symmetric  cycle  loss  to  improve  thequality of the generated caption and trace.

==> Localized Narratives/text/3.method.tex <==
\section{Method}

\begin{figure*}[!ht]
\centering
\includegraphics[width=0.95\textwidth]{Localized Narratives/figures/overall_architecture_pdf2.pdf} 
\caption{Overall architecture. Our proposed Mirrored Transformer (MITR) architecture effectively addresses the three tasks together by sharing most of the network modules. The structure is mirrored for processing the caption and trace. Depending on the task, we add a masking operation for the encoding/decoding of each module.}
\label{fig_overall_arc}
\end{figure*}
% In Section~\ref{subsection:define_3tasks}, we first introduce the three tasks proposed to model different relationships among the three modalities: image, caption and trace. 
% See Fig.~\ref{fig:three_tasks} for an illustration of the three tasks.
% In Section~\ref{subsection:mirrored_transformer}, we then introduce our network design which jointly models the three tasks. 
% In addition, we make those tasks interact with each other and get further gain.. \amy{This pragraph needs to be completed}

% \begin{figure}[!ht]
% \centering
% \includegraphics[width=0.42\textwidth]{Localized Narratives/figures/trace_to_bbox2.pdf} 
% \caption{Demonstration of how we map the trace segments to ground truth bounding boxes.}
% \label{fig:trace_to_bbox}
% \end{figure}
% Figure link: https://www.figma.com/file/pkgjSqGgpNXZoaOsMBKw3g/Localized-Narratives?node-id=0%3A1

\subsection{Three Tasks on the Three Modalities}
\label{subsection:define_3tasks}
We first introduce how we encode the new trace modality.
The trace is a series of points with corresponding timestamps, each associated with a single word from the caption.
Instead of encoding each individual point, we convert the trace into a sequence of word-aligned bounding boxes, i.e., one box per word.
This encoding mitigates the local ``drawing" variation (by different annotators) within the same region, and thus more reliably allows the model to attend to the full spatial extent of a referred region.


% Before defining the three vision-and-language modalities, we first must explain how we represent the mouse trace in each task. 
% Rather than considering each mouse point individually, we represent the trace as a sequence of caption-aligned bounding boxes (one box per word).
% We do this mapping for several reasons.
% First, for visual grounding, the ordering of the mouse points within a semantic region is not significant for generating a caption. In fact, as we see in Section~\ref{subsection:eval_metrics}, even the local ordering of entire trace bounding boxes does not necessarily affect the quality of the generated caption. 
% Second, it is useful for the model to attend to the full spatial extent of a referenced region, which a continuous mouse trace segment can help provide.

In order to generate this dense word-to-box alignment from the provided trace points, we take the following steps: 
% (see Fig.~\ref{fig:trace_to_bbox} for illustration):
($i$) Split the trace into segments, with one segment per word (using the word-to-trace alignment from Localized Narratives).
($ii$) Generate one bounding box per trace segment, by taking the axis-aligned minimum bounding box of the convex hull of the mouse points. Then we introduce the three tasks:
\paragraph{Controlled Trace Generation}
Given an image $I$ and a caption describing this image $\mathbf{w} =\{ w_1, w_2, \cdots, w_N \}$, the model is required to generate a trace indicating the visual grounding corresponding to the caption, in the form of an ordered region sequence $\mathbf{r}=\{r_1, r_2, \cdots, r_T\}$.

\paragraph{Controlled Caption Generation} 
Given an image $I$ and a mouse trace provided by the user that is mapped to a sequence of regions, $\mathbf{r}=\{r_1, r_2, \cdots, r_T\}$, the model generates a caption $\mathbf{w} =\{ w_1, w_2, \cdots, w_N \}$ describing the image along this trace. 

\paragraph{Joint Caption and Visual Trace Generation}
We further propose a task which can be regarded as an extension of standard image captioning: given an image $I$, the model generates both caption $\mathbf{w} =\{ w_1, w_2, ..., w_N \}$ and its corresponding trace of ordered regions $\mathbf{r}=\{r_1, r_2 ..., r_T\}$ that matches the caption. 

\subsection{Mirrored Transformer for Three Modalities}
\label{subsection:mirrored_transformer}

\begin{figure}[!ht]
\centering
\includegraphics[width=0.40\textwidth]{Localized Narratives/figures/Transformer_figure_pdf.pdf} % Reduce the figure size so that it is slightly narrower than the column.
% \vspace{-10pt}
\caption{Mirrored Transformer (\modelName) architecture. MHA stands for MultiHead Attention.}
\label{fig_transformer_arc}
% \vspace{-10pt}
\end{figure}
Although the three tasks defined above are quite different, they operate on the same set of three modalities: image, caption, and trace. 
In this work, we propose a model that effectively addresses all three tasks together in a unified framework with shared parameters, rather than building three separate models.
%leading to the possibility of getting benefits through joint training and bringing computational efficiency 
Due to its symmetric structure, we name this model architecture ``\textbf{MI}rrored \textbf{T}ransforme\textbf{R}" (\modelName), as in Fig.~\ref{fig_overall_arc}.
% Due to the flexibility of the mirrored design, our model can be easily extended to perform the task of controlled image captioning~\cite{cornia2019show}.

\paragraph{Features}
The inputs to the model are subsets of: image features, text features, and trace features. 
For image features, we use pre-trained Faster R-CNN~\cite{anderson2018bottom} to compute the visual features of the detected regions.
For the text feature, we sum up the positional embeddings and the word embeddings, as in~\cite{vaswani2017attention}, where the position refers to the index of the word within the caption. 
For the trace feature, we sum up the positional embeddings and the input trace, which is projected into $d$ hidden dimensions. 
Specifically, we define the trace position as the index of the  bounding box that is aligned with the word in the corresponding caption.
We denote the input visual features, text features, and trace features as $x_v, x_w, x_r$, respectively. 

\paragraph{Model Architecture}
As in Fig.~\ref{fig_transformer_arc}, our model is composed of three modules (corresponding to three modalities): image encoder, caption encoder-decoder, and trace encoder-decoder. 
Each module consists of a transformer with self-attention.
Specifically, the image encoder, $h_v$, is defined as:
\begin{equation}
\label{eq_h_v}
    h_v = \text{FFN}(\text{MultiHead}_v(x_v, x_v, x_v)),
\end{equation}
where we follow \cite{vaswani2017attention} to define the feed-forward network (FFN) as two linear transformation layers with a ReLU activation in between, and the MultiHead as:
\begin{equation}\nonumber
    \text{MultiHead}(Q,K,V) = \text{Concat}(\text{head}_1, ..., \text{head}_c)W^O
\end{equation}
\begin{equation}\nonumber
    \text{head}_i = \text{Attention}(QW_i^Q, KW_i^K,VW_i^V),
\end{equation}
where the projections are parameter matrices. 
We refer readers to \cite{vaswani2017attention} for additional details of MultiHead attention.
Note that there is no masking operation in the MultiHead module from Eqn.~\eqref{eq_h_v}, since we allow the model to attend to all visual features when processing the caption and trace.
% For consuming the information of caption and trace, we allow our model to see all visual features, thus no masking is applied in Equation~\eqref{eq_h_v}.

We then design a mirrored structure for the caption and trace modules, based on the observation that the two modalities are symmetric in the controlled caption generation and controlled trace generation tasks. 
%In the first task, the model generates a caption from the trace, and in the latter task the model generates a trace from the caption. 
The caption encoder-decoder, $h_w$, and trace encoder-decoder, $h_r$, are defined as:
\begin{equation}
\label{eq_h_w}\nonumber
    h_w = \text{MultiHead}_w^2(\text{MultiHead}_w^1(x_w,x_w,x_w), h_v, h_v)
\end{equation}
\begin{equation}
\label{eq_h_r}\nonumber
    h_r = \text{MultiHead}_r^2(\text{MultiHead}_r^1(x_r,x_r,x_r), h_v, h_v)
\end{equation}
%Depending on the specified task, 
Our caption and trace modules can switch roles between encoder and decoder seamlessly.
Inspired by~\cite{zhou2020unified}, this switching is implemented by a masking operation, where the encoder observes all inputs but the decoder only observes partial previous information.
This prevents the decoder from attending to future information. 
% We implement a masking operation in the first MultiHead modules in \eqref{eq_h_w} and \eqref{eq_h_r} (MultiHead$_w^1$ and MultiHead$_r^1$), depending on the specified task: 
We implement a masking operation in either MultiHead$_w^1$ or MultiHead$_r^1$, depending on the specified task: 
\begin{itemize}
    \setlength\itemsep{0em}
    \item For controlled caption generation, the input caption is shifted right by one position, and MultiHead$_w^1$ applies masking to prevent leftward information flow. This ensures every position can only see its previous positions in the attention module. Note, the input trace is not shifted and MultiHead$_r^1$ does not have any masking. 
    \item For controlled trace generation, the input trace is shifted right by one position and MultiHead$_r^1$ applies masking, while the input caption is not shifted and MultiHead$_w^1$ does not perform the mask operation.
    \item For the joint caption and trace generation task, both the input caption and input trace are shifted right by one position, and both MultiHead$_w^1$ and MultiHead$_r^1$ perform mask operations.
\end{itemize}

Our model also supports multiple layers.
The module between $x_v,x_w,x_r$ and $h_v,h_w,h_r$ can be repeated $N$ times. 
% Using the encoder and decoder terminology from \cite{vaswani2017attention}, which is frequently used in the literature, 
Specifically, MultiHead$_v$ acts as the encoder, while MultiHead$^1_w$, MultiHead$^2_w$, MultiHead$^1_r$, and MultiHead$^2_r$ switch roles between encoder and decoder depending on what task is being performed. 
All of these modules are shared across different tasks.

Finally, once $h_w$ and $h_r$ have been computed, MultiHead$^3_w$ and MultiHead$^3_r$ are used to fuse the information from caption and trace modules. 
Note that in the joint caption and trace generation task, both MultiHead$^3_w$ and MultiHead$^3_r$ need to include a mask operation, while in the other two tasks, no mask operation is needed.



\subsection{Controlled Trace Generation: Distance Score}
% Comment from Amy: I changed this subsection name slightly so that it will fit on one line
\label{subsection:eval_metrics}
Given a ground truth trace of length $q$, represented as a sequence of $q$ bounding boxes, and a predicted trace of length $m$, we need a score that can measure the distance between these two traces. 
When $q=m$, the most straightforward way is to compute the $L1$ loss between pairs of bounding boxes (where the two bounding boxes at the same index in the sequence form a pair):
$D(\mathbf{r}^{gt}, \hat{\mathbf{r}}) = \frac{1}{q}\sum_{i=1}^{q} | r_i^{gt} - \hat{r_i} |$,
where $|r_i^{gt} - \hat{r_i} |$ is the mean $L1$ distance on the four coordinates of the $i$-th bounding box.

However, there are two main challenges. 
First, when $q\neq m$, we need to find the exact alignment between the two sets of bounding boxes. 
Second, even when $q=m$, we may not want to force the two sets to match in the given order because the dataset may contain examples where the local bounding box ordering is not semantically meaningful. 
% For example, an annotator may use several words to describe an entire object (e.g., ``the large black cat"), which is distinct from the case where an annotator uses separate words to reference visually distinct components of a single object (e.g., ``the cat has green eyes and a long tail"). 
% The ordering of the words/bounding boxes matters for the second case (we do not want to attend to ``tail" when the annotator is describing the cat's eyes), but it does not matter for the first case. 
% Therefore, we do not want to penalize a model that predicts a different local bounding box ordering for the first case.
% \Amy{removed the above sentences I wrote because we are over-length anyway, and I think the second problem is self-evident without needing an example}
% There are some literature works providing a mechanism to approach this question. 
\cite{chakraborty2017geometric} shows that if we treat each ``trajectory'' as a sequence of 
points on a Riemannian manifold,
a distance metric between two trajectories can be derived on a homogeneous space. 
Such an idea is useful for the case where the sample dimension is much larger than the number of samples. 
In our case, the sample dimension is small (4-D vector to represent each bounding box), so we choose to simply cast the evaluation task as a simple bipartite matching problem.
%To address the two issues, we cast the evaluation task into a bipartite matching problem. 
Note that standard bipartite matching is not a direct solution as it operates on two unordered sets of samples, ignoring the ordering within a trace. 
Instead, we propose to add local constraints to the bipartite matching so that the orderless matching can only happen within a local window. 
% This resolves the two challenges mentioned above at the same time: 
On the one hand, it provides a way to match two ordered sequences of bounding boxes; on the other hand, it allows local disorder, which is robust to the noise in the dataset annotation.

Consider two traces of lengths $q$ and $m$; without loss of generality, we assume that $q \leq m$. 
Let $C\in \mathbb{R}^{q\times m}$ be the cost matrix where $C_{ij}$ is the mean $L1$ distance between the four coordinates of the $i$-th box from the first trace and $j$-th box from the second trace, and let $X$ be the assignment matrix. 
We solve the following linear programming problem to get the distance between these two traces:
\begin{align*}
    \min_X \quad &\Tr (CX^T) \\
    s.t., \quad & X\mathbf{1}_m = \mathbf{1}_q,\quad  X^T\mathbf{1}_q \leq \mathbf{1}_m,\quad X\geq 0, \quad X_{i,j} = 0,\\
    &\forall i,j \quad s.t., \quad 0\leq i\leq q-1,\quad 0\leq j \leq m-1,\\ &j<\floor*{(i-k)\frac{m}{q}} \quad \text{or}  \quad  j \geq (i+1+k)\frac{m}{q},
\end{align*}
where $\mathbf{1}_m\in \mathbb{R}^{m}$ is all one vector and $k$ is the window size controlling the local range of disordered matching. 
For example, when $q=m$ and $k=1$, this allows one box from the first trace to match with the box at the same index from the second trace and also its left and right neighbors. 
After solving this linear programming problem, we use $\text{Tr}(CX^T) / q$ as the distance score between two traces. 
We call our proposed score the Local Bipartite Matching score (LBM). {In addition to using this as an evaluation measure, one 
could further incorporate this score into training to learn traces for a better matching score, by utilizing recently proposed differentiable linear programming solvers \cite{meng2020physarum,agrawal2019differentiable}. To keep the presentation succinct, we do not discuss these extensions in this paper.}


\subsection{Cycle Interaction of Trace and Caption}
% During the training of controlled caption generation, the input is always the annotation trace from the Localized Narratives dataset, where most images only have one annotated trace with the associated caption (a small portion of them have five annotations, due to annotator replication). 
% However, the model should be able to generate a caption given any meaningful trace that is not too unsmooth. 
% Under this assumption, and the fact that the controlled caption generation and our proposed controlled trace generation are inverse tasks, we propose to randomly permute the trace and then send it to the controlled caption generation model. 
Another interesting finding of our model architecture is that the controlled trace generation and controlled caption generation are dual problems in one framework, i.e., the output of one direction serves as the input of the other.
This inspires us to allow the two modules interact with each other.
First, we randomly permute the trace and feed it into the controlled caption generation module, generating the caption.
Then, we feed this generated caption\footnote{Gumbel-softmax~\cite{jang2016categorical} is applied to approximate the non-differentiable categorical sampling of words.} into our controlled trace generation model and enforce that the predicted trace be close to the originally permuted trace by adding a cycle loss. 
By doing so, we enrich the training set by adding more meaningful but unseen trace-caption pairs. 
As shown in Section~\ref{subsection:cycle_loss}, this further boosts the performance of both tasks.

We denote our mirrored transformer model as $f()$, the controlled trace generation task as $\hat{\mathbf{r}}=f(I, \mathbf{w})$, and the controlled caption generation task as $\hat{\mathbf{w}} = f(I, \mathbf{r})$. 
We enforce the cycle consistency via
% \begin{equation}
%     L_{\mathbf{w}\to \mathbf{\hat{r}}\to \mathbf{\hat{w}}} =  \text{Dist}_\mathbf{w}(f(I, f(I,\mathbf{w})), \mathbf{w})
% \end{equation}
% and 
\begin{equation}\label{eq:cycle_loss}\nonumber
    L_{\mathbf{\Tilde{r}}\to \mathbf{\hat{w}}\to \mathbf{\hat{r}}} =  \text{Dist}_{\mathbf{r}}(f(I, f(I,\mathbf{\Tilde{r}})), \mathbf{\Tilde{r}}),
\end{equation}
where $\text{Dist}_\mathbf{r}$ is the $L1$ loss between the predicted trace and the ground truth trace, and $\mathbf{\Tilde{r}}$ is the randomly manipulated trace. 
Specifically, we perform two types of manipulation: ($i$) randomly switch the trace within a mini-batch, and ($ii$) cut a trace into $S$ segments and randomly permute these segments to form a new trace.
We show that both manipulations are effective in improving the performance.

\subsection{Total Loss Function}
\label{subsec:total_loss}
The final loss function can be formulated as:
\begin{align}\label{eq:total_loss}
     L_{\text{total}} & = \lambda_1 L_{\text{[trace]}} + \lambda_2 L_{\text{[caption]}}\nonumber \\
     &+ \lambda_3 L_{\mathbf{\Tilde{r}}\to \mathbf{\hat{w}}\to \mathbf{\hat{r}}} + \lambda_4 L_{\text{[joint]}},
\end{align}
where $L_{[\text{trace}]}$ is the $L1$ loss between the predicted trace boxes and ground truth trace boxes for controlled trace generation, $L_{[\text{caption}]}$ is the cross-entropy loss of the caption for controlled caption generation, $L_{\mathbf{\Tilde{r}}\to \mathbf{\hat{w}}\to \mathbf{\hat{r}}}$ is the cycle loss, and $L_{\text{[joint]}}$ is the sum of the trace loss and the caption loss for the joint caption and trace generation task. 
% If a task is not used, we simply set its $\lambda$ to be zero.

%When feeding $\mathbf{\hat{w}}$ as the input caption into the controlled trace generation network, we need to make it differentiable, so we cannot discretize the output logits into discrete tokens. Here, we use the Gumbel-Softmax \cite{jang2016categorical} to do the categorical reparameterization. This enables us to compute backward gradients from the sampled caption that is drawn from the categorical distribution described by the output logits of the controlled caption generation network, before it is discretized into $\mathbf{\hat{w}}$. 



\subsection{Bridging the Gap between Training and Testing}
Discrepancies between training and inference always exist in sequential prediction models~ \cite{bengio2015scheduled}. At training, the ground-truth input/output trace at each time step is provided, while at inference the unknown previous trace is replaced by a trace generated by the model itself.

In our proposed joint caption and trace generation task, such discrepancies are even more severe than in standard caption generation, as both the previous word and trace box are generated by the model and thus are connected.
% Especially, trace generation suffers more from noise because the previous words largely determine the current word, while the trace could quickly move to anywhere in the image following the current word. 
The generated trace especially suffers from noise because, unlike the caption, the trace lacks syntax.
A single offset could cause the following trace boxes to quickly move to anywhere in the image.
To alleviate this problem, we propose a random replacement of the input trace boxes, where we replace a box with $[0,0,1,1,1]$ (corresponding to the whole image) with probability $p$. As shown in Table~\ref{tab:task3}, this approach improves the performance of joint caption and trace generation by a clear margin. 
% while avoiding extra computation overhead like the one in \cite{bengio2015scheduled}.





==> Localized Narratives/text/4.experiments.tex <==
\section{Experiments}
\subsection{Dataset}

\begin{table}
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    \scalebox{0.95}{
    \begin{tabular}{l | c c c}
        \thickhline
         & \# images & \# captions & \# words/capt \\
        % \hline 
        % COCO Captions~\cite{chen2015microsoft} & 123,287 & 616,767 & 10.5 \\
        \hline
        COCO Loc. Narr. \cite{pont2019connecting} & 123,287 & 142,845 & 41.8 \\
        \hline
        Flickr30k Loc. Narr. \cite{pont2019connecting} & 31,783 & 32,578 & 57.1 \\
        \hline
        ADE20k Loc. Narr. \cite{pont2019connecting} & 22,210 & 22,529 & 43.0 \\
        \hline
        Open Images Loc. Narr. \cite{pont2019connecting} & 671,469 & 675,155 & 34.2 \\
        \hline
        \thickhline
        % COCO & val & 5,000 & 8,573 & 40.4 \\
        % \hline
        % Open Images & train & 504,413 & 507,444 & 35.5 \\
        % & val & 41,620 & 41,691 & 29.9 \\
        % & test & 125,436 & 126,020 & 30.6 \\
        %\hline
        % Flickr30k & train & 29,783 & 30,546 & 57.1 \\
        % & val & 1,000 & 1,009 & 57.0 \\
        % & test & 1,000 & 1,023 & 57.6 \\
        % \hline
        % ADE20k & train & 20,210 & 20,476 & 42.9 \\
        % & val & 2,000 & 2,053 & 43.9 \\
    \end{tabular}
    }
    % \caption{Information for the datasets we evaluate on. The grounding for COCO Captions (row 1) is whole caption $\rightarrow$ whole image. For COCO annotated with the Localized Narratives framework (row 2), the grounding is individual word $\rightarrow$ region. There are more captions than the the images due to some multi-review annotation.}
    \caption{Localized Narratives built on top of COCO, Flickr30k, ADE20k, and Open Images.}
    \label{tab:datasets}
\end{table}
% Note: I found the average caption length for all of COCO - Localized Narratives by doing a weighted average of the average train and val caption length:
% ((134272/142845)*41.9) + ((8473/142845)*40.4) = 41.8

We conduct experiments on four datasets: COCO, Flickr30k, ADE20k, and Open Images, with annotations from two different frameworks: COCO Captions~\cite{chen2015microsoft} and Localized Narratives~\cite{pont2019connecting}, summarized in Table~\ref{tab:datasets}. We perform an ablation study on COCO and report the performance of our best performing model on the other three datasets in Localized Narratives and the downstream task introduced in Section~\ref{subsection:downstream_tasks} (evaluated on the COCO Captions annotations). We use the COCO2017 split for all experiments except Section~\ref{subsection:downstream_tasks}, where we follow \cite{cornia2019show} to use the split they provide. 

The annotations provided by Localized Narratives are challenging to work with for a number of reasons.
First, the human-generated trace segment $\mathbf{r}_i$ is a noisy visual representation of the mentioned object, due to imperfect voice-trace synchronization (e.g., if the annotator moves their mouse without speaking), errors in voice-word synchronization (from the automatic sequence-to-sequence alignment model in~\cite{pont2019connecting}), inconsistent drawing habits among annotators, and the different nature of mouse trace lines vs. bounding boxes. 
Second, not every word can be meaningfully grounded in the image, such as existentials (e.g., ``there are") and language referring to the observer (e.g., ``in this image, I can see ..."). By our estimate, such words account for at least 20\% of the words in the COCO validation captions from Localized Narratives. Traces for such words are less meaningful than the other groundable words. 


\begin{table*}[!ht]
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    \resizebox{1.5\columnwidth}{!}{
    \begin{tabular}{l l | c c c c c c }
        \thickhline
        Method & Trained on & BLEU-1 & BLEU-4 & METEOR & ROUGE$_L$ & CIDEr & SPICE \\
        \hline 
        \cite{pont2019connecting} & Task2 & 0.522 & 0.246 & N/A & 0.483 & 1.065 & 0.365 \\
        \hline
        Baseline & Task2 & 0.563  & 0.255 & 0.240 & 0.453 & 0.997 &0.293 \ \\
        \modelName & Task2 & 0.577 & 0.257 & 0.245 & 0.456 & 1.213 & 0.293 \\
        \modelName & Task2 + Task1 & 0.586 & 0.272 & 0.252 & 0.470 & 1.329 & 0.307 \\
        \modelName & Task2 + Task1 + cycle$_s$ & 0.596 & 0.282 & 0.257 & 0.476 & 1.390 & 0.309 \\
        \modelName & Task2 + Task1 + cycle$_b$ & 0.598 & 0.286 & 0.258 & 0.479 & 1.407 & 0.313 \\
        \modelName(2 layer) & Task2 + Task1 + cycle$_b$ & \textbf{0.607} & \textbf{0.292} & \textbf{0.263} & \textbf{0.487} & \textbf{1.485} & \textbf{0.317} \\
        \thickhline
    \end{tabular}
    }
    \caption{Quantitative results for Task 2 (controlled caption generation) on COCO. cycle$_s$ and cycle$_b$ refer to two types of cycle loss defined in Sec~\ref{subsection:cycle_loss}. Results from \cite{pont2019connecting} are not directly comparable to ours due to differences mentioned in Sec~\ref{subsec:individual_tasks}.}
    \label{tab:task2}
\end{table*}

\begin{table*}[!ht]
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    \resizebox{1.95\columnwidth}{!}{
    \begin{tabular}{l l | c c c c c c c c}
        \thickhline
        Method & Trained on & BLEU-1 & BLEU-4 & METEOR & ROUGE$_L$ & CIDEr & SPICE & LBM(k=0) & LBM(k=1) \\
        \hline 
        Baseline & Task2 & 0.355 & 0.087 & 0.155 & 0.307 & \textbf{0.310} & 0.210 & N/A & N/A \\
        \modelName & Task3 & 0.387 & 0.118 & 0.168 & 0.316 & 0.170 & 0.194 & 0.387 & 0.369 \ \\
        \modelName & Task3 + random mask & 0.395 & \textbf{0.128} & \textbf{0.184} & \textbf{0.328} & 0.219 & \textbf{0.223} & 0.308 & 0.292 \\
        \modelName & Task3 + Task1 + Task2 + random mask & \textbf{0.417} & 0.125 & 0.178 & 0.323 & 0.216 & 0.213 & \textbf{0.283} & \textbf{0.267} \\
        \thickhline
    \end{tabular}
    }
    \caption{Quantitative results for Task 3 (joint caption and trace generation) on COCO.}
    \label{tab:task3}
\end{table*}


\begin{table*}[!ht]
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    \resizebox{1.95\columnwidth}{!}{
    \begin{tabular}{l l l| c c c c c c c c}
        \thickhline
        Dataset & Method & Trained on & BLEU-1 & BLEU-4 & METEOR & ROUGE$_L$ & CIDEr & SPICE & LBM(k=0) & LBM(k=1) \\
        \hline 
        Flickr30k & Baseline & Task1& N/A & N/A & N/A & N/A & N/A & N/A & 0.253 & 0.249\\
        Flickr30k & Baseline & Task2 & 0.620 & 0.345 & 0.286 & 0.524 & 1.763 & 0.341 & N/A & N/A\\
        Flickr30k & \modelName & Task1 + Task2 + cycle$_b$ &   \textbf{0.644} & \textbf{0.374} & \textbf{0.300} & \textbf{0.547} & \textbf{2.014} & 0.365 & 0.195 & 0.188\\
        Flickr30k & \modelName(2 layer) & Task1 + Task2 + cycle$_b$ & 0.640 & 0.366 & 0.297 & 0.543 & 2.000 & \textbf{0.374} & \textbf{0.183} & \textbf{0.176}  \\
        \hline
        ADE20k & Baseline & Task1 & N/A & N/A & N/A & N/A & N/A & N/A & 0.251 & 0.247\\
        ADE20k & Baseline & Task2 & 0.565 & 0.278 & 0.259 & 0.475 & 1.288 & 0.341 & N/A & N/A\\
        ADE20k & \modelName & Task1 + Task2 + cycle$_b$ & \textbf{0.580} & \textbf{0.297} & \textbf{0.269} & \textbf{0.490} & \textbf{1.463} & 0.354  & \textbf{0.177} & \textbf{0.168}\\
        ADE20k & \modelName(2 layer)  & Task1 + Task2 + cycle$_b$ & 0.575 & 0.292 & 0.267 & 0.490 & 1.437 & \textbf{0.358} & 0.191 & 0.185 \\
        \hline
        Open Images & Baseline & Task1 & N/A & N/A & N/A & N/A & N/A & N/A & 0.212 & 0.209 \\
        Open Images & Baseline & Task2 & 0.560 & 0.273 & 0.261 & 0.503 & 1.467 & 0.361 & N/A & N/A \\
        Open Images & \modelName & Task1 + Task2 + cycle$_b$ & 0.573 & 0.292 & 0.271 & 0.520 & 1.584 & 0.372 & \textbf{0.180} & \textbf{0.171} \\
        Open Images & \modelName(2 layer)  & Task1 + Task2 + cycle$_b$ & \textbf{0.584} & \textbf{0.308} & \textbf{0.276} & \textbf{0.531} & \textbf{1.887} & \textbf{0.381} & 0.211 & 0.206  \\
        
        \thickhline
    \end{tabular}
    }
    \caption{Quantitative results for Task 1 and Task2 on Localized Narratives of Flickr30k, ADE20k and Open Images.}
    \label{tab:task1_2_three_datasets}
\end{table*}


% \begin{table*}[!ht]
%     \centering
%     \small
%     \setlength{\tabcolsep}{4pt}
%     \resizebox{1.84\columnwidth}{!}{
%     \begin{tabular}{l l l| c c c c c c c c}
%         \thickhline
%         Dataset & Method & Trained on & BLEU-1 & BLEU-4 & METEOR & ROUGE_L & CIDEr & SPICE & LBM(k=0) & LBM(k=1) \\
%         \hline 
%         Flickr30k & Baseline & Task2 \\
%         Flickr30k & \modelName & Task3 + random mask &  \\
%         \hline
%         ADE20k & Baseline & Task2 \\
%         ADE20k & \modelName & Task3 + random mask &  \\
%         \hline
%         Open Images & Baseline & Task2 \\
%         Open Images & \modelName & Task3 + random mask &  \\
        
%         \thickhline
%     \end{tabular}
%     }
%     \caption{Quantitative results for Task 3 on Localized Narratives of Flickr30k, ADE20k and Open Images.}
%     \label{tab:task3_three_datasets}
% \end{table*}


\subsection{Experimental Setting}
\label{subsec:exp_setting}
We use our mirrored transformer (\modelName) defined in Section~\ref{subsection:mirrored_transformer} with $N=1$ (as shown in Fig.~\ref{fig_transformer_arc}). The hidden size of attention layers is $512$ and that of the feed-forward layers is $2048$. We train the network with batch size $30$ using the Adam optimizer \cite{kingma2014adam}. The initial learning rate is $5\mathrm{e}{-4}$, which decays every $3$ epochs with decay rate $0.8$, for a total of $30$ epochs. We use the same training setup for all experiments reported in this paper. The random masking rate for joint caption and trace prediction is $p=0.5$. In the following, we denote controlled trace generation as Task$1$, controlled caption generation as Task$2$, and joint caption and trace generation as Task$3$. 
% For joint training of Task1 and Task2, we set $\lambda_1=1$, $\lambda_2=0.3$, $\lambda_3=\lambda_4=0$. For joint training of Task1 and Task2 with cycle loss, we use $\lambda_1=1$, $\lambda_2=0.3$, $\lambda_3=0.1$, $\lambda_4=0$. For joint training of Task1, Task2, and Task3, we set $\lambda_1=\lambda_2=\lambda_4=1$, $\lambda_3=0$.

\paragraph{Controlled Trace Generation}
In this task, we represent the trace as an ordered sequence of bounding boxes, and the model predicts one bounding box for each word of the input caption, as described in Section~\ref{subsection:define_3tasks}. Given a ground truth trace $\mathbf{r}^{gt}=\{r_1^{gt}, r_2^{gt}, ..., r_T^{gt}\}$ and a predicted trace $\mathbf{\hat{r}}=\{\hat{r}_1, \hat{r}_2, ..., \hat{r}_T\}$ for the same image,  we compute the local bipartite matching (LBM) score proposed in Section~\ref{subsection:eval_metrics} for $k=0$ and $k=1$. 

\paragraph{Controlled Caption Generation}
Given an image and a trace, the model predicts the caption corresponding to the trace. When evaluating the quality of generated captions, we report the following widely adopted metrics: BLEU-$1$, BLEU-$4$ \cite{BLEU}, METEOR \cite{METEOR}, ROGUE \cite{ROUGE}, CIDEr \cite{CIDEr}, SPICE \cite{SPICE}.
%and EMD \cite{EMD}. 
We use beam search with size $5$. 

\paragraph{Joint Caption and Trace Generation} In this task, the model is given only an image as input and outputs both caption and trace simultaneously. The model produces outputs iteratively, generating one word and one corresponding bounding box at each time step. At test time, we end the generation when the caption generation branch outputs the \texttt{END} token. In this process, since the model itself controls the length of the output, the length of the predicted trace $\mathbf{\hat{r}}$ may differ from the length of the ground truth trace $\mathbf{r}^{gt}$. The max length for generating caption and trace is set to be $100$. We report our LBM metric for both $k=0$ and $k=1$. 

\paragraph{Baselines}
For controlled trace generation, we construct the baseline by using a standard one-layer encoder-decoder transformer architecture as defined in \cite{vaswani2017attention} and feed both visual features and captions to the encoder. Similarly, for controlled caption generation, we use the same architecture as a baseline and feed both visual features and traces to the encoder. For joint caption and trace generation, we construct the baseline by also using the same architecture, but only using visual features as input, and we train it on the caption generation task.

\subsection{Results on Individual Tasks}
\label{subsec:individual_tasks}
\paragraph{Controlled Trace Generation} In Fig.~\ref{fig:qual_results_tasks_1_2_coco} (left), we demonstrate the qualitative results of the controlled trace generation: we can see that the trace closely follows the ground truth trace and also semantically corresponds well to the input caption. Table \ref{tab:task1} shows the quantitative results. 
From the table, we see that our proposed MITR outperforms the baseline method constructed in Section~\ref{subsec:exp_setting} (standard transformer with one encoder and one decoder \cite{vaswani2017attention}). 

\begin{table}[!ht]
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    \resizebox{1.0\columnwidth}{!}{
    \begin{tabular}{l l | c c }
        \thickhline
        Method & Trained on & LBM (k=0) & LBM (k=1) \\
        \hline 
        Baseline & Task1 & 0.208 & 0.204 \\
        \modelName & Task1 & 0.171  & 0.159 \\
        \modelName & Task1 + Task2 & 0.169 & 0.157 \\
        \modelName & Task1 + Task2 + cycle$_s$ & 0.165 & 0.156 \\
        \modelName & Task1 + Task2 + cycle$_b$ & 0.166 & 0.155 \\
        \modelName (2 layer) & Task1 + Task2 + cycle$_b$ & \textbf{0.163} & \textbf{0.154} \\
        \thickhline
    \end{tabular}
    }
    \caption{Quantitative results for Task 1 (controlled trace generation). cycle$_s$ and cycle$_b$ refer to the two cycle losses defined in Sec~\ref{subsection:cycle_loss}. Note: smaller values of LBM are better.}
    \label{tab:task1}
\end{table}




\begin{figure*}[!ht]
\centering
\includegraphics[width=0.88\textwidth]{figures/COCO_Tasks_1_and_2.pdf} 
% \vspace{-10pt}
\caption{Qualitative results on Tasks 1 and 2 on COCO. (See supplement for visualizations for other three datasets)}
\label{fig:qual_results_tasks_1_2_coco}
% \vspace{-10pt}
\end{figure*}


\begin{figure*}[!ht]
\centering
\includegraphics[width=0.88\textwidth]{figures/COCO_Tasks_3.pdf} 
% \vspace{-10pt}
\caption{Qualitative results on Task 3 on COCO.}
\label{fig:qual_results_tasks_3_coco}
% \vspace{-10pt}
\end{figure*}

% \begin{figure*}[!ht]
% \centering
% \includegraphics[width=0.88\textwidth]{figures/Qualitative_results_Tasks_1_2_3_two_rows.pdf} 
% % \vspace{-10pt}
% \caption{Qualitative results on Tasks 1, 2, and 3 (with more results in the supplementary file).}
% \label{fig:qual_results_tasks_1_2_3}
% % \vspace{-10pt}
% \end{figure*}
% Figure link: https://www.figma.com/file/pkgjSqGgpNXZoaOsMBKw3g/Localized-Narratives?node-id=0%3A



\paragraph{Controlled Caption Generation}  
We show our quantitative results in Table~\ref{tab:task2} and qualitative results on the right side in Fig.~\ref{fig:qual_results_tasks_1_2_coco}. 
Our baseline model differs from the one in \cite{pont2019connecting} in several places: 
we use a one-layer encoder-decoder transformer while \cite{pont2019connecting} uses two layers;
% we use the region features provided by \cite{anderson2018bottom} which contain features of $10$-$100$ boxes per image while \cite{pont2019connecting} extracted top-$16$ boxes. 
in addition, we process the trace by cutting the trace by word while \cite{pont2019connecting} cuts the trace by a fixed time interval. 
Thus, results from \cite{pont2019connecting} are not directly comparable to ours. 
We mention the performance of \cite{pont2019connecting} in Table \ref{tab:task2} for easy reference.

%\ning{Here, we need to explain more how our baseline is different from \cite{pont2019connecting}}


\paragraph{Joint Caption and Trace Generation} The quantitative results for this task are in Table~\ref{tab:task3}. We can see that by modeling the trace at the same time as the caption, the performance of caption generation improves by a large margin over the baseline, which only models the caption. In addition, our proposed random masking technique further improves the performance of Task 3 on caption generation by over $1\%$ absolute improvement on all metrics, and on trace generation by nearly $20\%$ relative improvement. The qualitative results are shown in Fig.~\ref{fig:qual_results_tasks_3_coco}. Without human annotated attention traces to guide the caption generation, sometimes the same objects or descriptions are repeated multiple times in a single caption. 
This suggests that future developments must keep an account of all the objects referenced to avoid repetition.


\subsection{Joint Training Results}
We demonstrate that, by performing joint training, our model can boost the performance of each individual task while using approximately one half of the parameters and training compute cost, compared with training one separate model for each individual task. The quantitative results are in Tables~\ref{tab:task1} and~\ref{tab:task2}. 
Further, we can see from Table \ref{tab:task3} that the joint training of Task 1 and Task 2 can also help Task 3. 


\subsection{Cycle Loss Results}
\label{subsection:cycle_loss}
We show that, by enforcing cycle consistency, both controlled trace generation and controlled caption generation are further improved when joint training is used. The quantitative results are in Tables~\ref{tab:task1} and \ref{tab:task2}. We use cycle$_s$ to represent cycle loss where a single trace is cut into segments and then randomly permuted before forming a new trace, and cycle$_b$ to represent cycle loss where the trace is permuted along the batch dimension within a mini-batch. Adding cycle$_b$ achieves over $1\%$ absolute improvement on BLEU-1 and BLEU-4 compared with our joint training result and over $3\%$ absolute improvement from our baseline model.

\subsection{Results on Flickr30k, ADE20k, Open Images} 
\label{subsection:three_datasets}
We also report the performance of our best performing model and the baseline model on another three datasets (Flickr30k, AED20k, Open Images), where Localized Narratives are also collected~\cite{pont2019connecting}. 
The results are given in Table \ref{tab:task1_2_three_datasets}. 
As shown, our method achieves consistent improvement over the baseline methods on all datasets.

\begin{table}[!h]
    \centering
    \small
    \setlength{\tabcolsep}{4pt}
    \scalebox{0.95}{
    \begin{tabular}{l | c c c c c c }
        \thickhline
          & B-1 & B-4 & M & R & C & S \\
        \hline 
        Ours \emph{w/o} pretrain & 0.463  & 0.182 & 0.219 & 0.466 & 1.746 & 0.363 \ \\
        Ours \emph{w/} pretrain  & \textbf{0.474} & \textbf{0.189} & \textbf{0.225} & \textbf{0.475} & \textbf{1.819} & \textbf{0.370} \\
        \thickhline
    \end{tabular}
    }
    \caption{Downstream task on guided caption generation.}
    \label{tab:task_downstream}
\end{table}

\subsection{Downstream Task}
\label{subsection:downstream_tasks}
We further investigate the benefit of our joint training framework. 
By pre-training using our joint training framework on Localized Narratives \cite{pont2019connecting} and fine-tuning on a guided caption generation task \cite{cornia2019show} on COCO Captions~\cite{chen2015microsoft}, we are able to get better results than directly training on COCO Captions. 
In this experiment, we follow~\cite{cornia2019show} to use the COCO split provided by~\cite{karpathy2015deep}.

The task is defined as: given an image $I$ and a sequence of ordered bounding boxes $\mathbf{r}=\{r_1, r_2,\cdots, r_T\}$ as guidance, the model generates a caption $\mathbf{w} =\{ w_1, w_2, \cdots, w_N \}$. This task is similar to our controlled caption generation task (Task 2), but we do not assume any correspondence between the boxes and words for both training and testing. 
Note that \cite{cornia2019show} considers a slightly different setting, where the dense correspondences between boxes and words are given during training but not at testing.
Thus a special gate function was proposed to automatically attend the words to the boxes during test time.  
See the supplementary material for more details. 
The results are in Table~\ref{tab:task_downstream}, where pre-training offers a clear gain.


% \begin{figure}[!ht]
% \centering
% \includegraphics[width=0.5\textwidth]{figures/Qualitative_results_task_3.pdf} % Reduce the figure size so that it is slightly narrower than the column.
% % \vspace{-10pt}
% \caption{Qualitative results on Task 3.}
% \label{fig:qual_results_task_3}
% % \vspace{-10pt}
% \end{figure}
% % Figure link: https://www.figma.com/file/pkgjSqGgpNXZoaOsMBKw3g/Localized-Narratives?node-id=0%3A

==> Localized Narratives/text/5.conclusion.tex <==
\section{Conclusion}
We presented a unified framework for modeling vision, language, and human attention traces.
Our work is built on top of the Localized Narratives framework and motivated by the need for longform image captions and dense visual grounding.
We proposed a Mirrored Transformer model architecture that was jointly trained on three vision-and-language tasks.
We demonstrated the effectiveness of our approach through detailed experiments on four datasets.

